A Basic Modal Logic for the Abstract Treatment of Quantum Mixed States

Quantum logic has developed in various directions since its inception. However, many existing logical approaches either focus only on pure states, or use Hilbert-space models in which the abstract relationship between pure states, mixed states, and probabilities is not made explicit. In this work, we introduce a model designed to handle quantum mixed states abstractly. Furthermore, we construct a proof system for the proposed logic and establish its completeness with respect to the intended semantics.

==> eptcsdata.tex <==
\providecommand{\firstpage}{32}
\providecommand{\publicationstatus}{A. Indrzejczak, T. Jarmu\.zek, M. Klonowski, \& M. Zawidzki (Eds.):\\ Twelfth International Conference on\\ Non-Classical Logics. Theory and Applications (NCL'26)\\
EPTCS 455, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.455.4}{10.4204/EPTCS.455.4}}
\pdfoutput=1

